Combining reconstruction and edge detection in computed tomography

We present two methods that combine image reconstruction and edge detection in computed tomography (CT) scans. Our first method is as an extension of the prominent filtered backprojection algorithm. In our second method we employ $\ell^{1}$-regularization for stable calculation of the gradient. As opposed to the first method, we show that this approach is able to compensate for undersampled CT data.

==> BVM-Paper - arXiv/commands.tex <==
% colon centering alogn the equals-sign
\mathchardef\ordinarycolon\mathcode`\:
\mathcode`\:=\string"8000\def\R{\mathbb{R}}
\begingroup \catcode`\:=\active\def\Z{\mathbb{Z}}
  \gdef:{\mathrel{\mathop\ordinarycolon}}\def\N{\mathbb{N}}
\endgroup

% mathbb letters
\newcommand{\K}{\mathbb{K}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\renewcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}

\usepackage{mathtools}
\usepackage{mathrsfs}
%----- Mathscript ------
\newcommand{\Am}{\mathscr{A}}
\newcommand{\Bm}{\mathscr{B}}
\newcommand{\Cm}{\mathscr{C}}
\newcommand{\Em}{\mathscr{E}}
\newcommand{\Fm}{\mathscr{F}}
\newcommand{\Gm}{\mathscr{G}}
\newcommand{\Hm}{\mathscr{H}}
\newcommand{\Jm}{\mathscr{J}}
\newcommand{\Mm}{\mathscr{M}}
\newcommand{\Km}{\mathscr{K}}
\newcommand{\Nm}{\mathscr{N}}
\newcommand{\Um}{\mathscr{U}}
\newcommand{\Pm}{\mathscr{P}}
\newcommand{\Om}{\mathscr{O}}
\newcommand{\Sm}{\mathscr{S}}
\newcommand{\Tm}{\mathscr{T}}

%--------------------
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}

%----------- New Math. Symbols ------------
\newcommand{\bdot}{\boldsymbol{\cdot}}                % Mittelgr. zentralerPunkt
%\newcommand{\varprod}{\mathop{\vcenter{\hbox{\Huge $\times$}}}}  
\newcommand{\id}{\mathrm{id}} 						  %      
\newcommand{\g}{\mathrm{g}} 
\newcommand{\WF}{\mathrm{WF}}                         % Wavefront set
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}      % Norm
\newcommand{\anorm}[1]{|\!|\!|#1|\!|\!|}              % Norm
\newcommand{\abs}[1]{\left|#1\right|}                 % Absolutbetrag
\newcommand{\paren}[1]{\left(#1\right)}               % Klammern
\newcommand{\bparen}[1]{\left[#1\right]}               % eckige Klammern
\newcommand{\sparen}[1]{\left\{#1\right\}}		      % Mengenklammer
\newcommand{\sqparen}[1]{\left[#1\right]}             % eckige Klammern
\newcommand{\h}[1]{\left\langle#1\right\rangle}       % Skalarprodukt
\newcommand{\lin}[1]{\mathrm{span}\left(#1\right)}  % lineare H"ulle
\newcommand{\clin}[1]{\overline{\lin{#1}}}            % abgeschl. lin. H"ulle
\newcommand{\mc}[2]{\omega_{#1}(#2)}                  % Glattheitsmodul
\newcommand{\ran}[1]{\mathrm{ran}\left(#1\right)}     % range
\newcommand{\dom}[1]{\mathrm{dom}\left(#1\right)}     % domain
\newcommand{\floor}[1]{\left.\lfloor #1\rfloor\right.}
\newcommand{\ceil}[1]{\left.\lceil #1\rceil\right.}
\renewcommand{\ker}[1]{\mathrm{ker}\left(#1\right)}   % kernel
\renewcommand{\d}{\,\mathrm{d}}						  % within the integral sign
\newcommand{\conv}{\ast}
\DeclareMathOperator*{\supp}{\mathrm{supp}}           % support
\DeclareMathOperator*{\singsupp}{\mathrm{sing\:supp}} % singular support
\DeclareMathOperator*{\sinc}{\mathrm{sinc}}           %
\DeclareMathOperator*{\sgn}{\mathrm{sgn}}
\DeclareMathOperator*{\Sgn}{\mathrm{Sgn}}
\DeclareMathOperator*{\esssup}{\mathrm{ess\:sup}}
\DeclareMathOperator*{\argmax}{\mathrm{arg\:max}}
\DeclareMathOperator*{\argmin}{\mathrm{arg\:min}}
\DeclareMathOperator*{\grad}{\mathrm{grad}}
\DeclareMathOperator*{\Si}{\mathrm{Si}} % Sine integral
\DeclareMathOperator{\arcsec}{arcsec}
\DeclareMathOperator{\arccot}{arccot}
\DeclareMathOperator{\arsinh}{arsinh}
\DeclareMathOperator{\arcosh}{arcosh}
\DeclareMathOperator{\artanh}{artanh}
\DeclareMathOperator{\arcoth}{arcoth}
\renewcommand{\Re}{\mathrm{Re}}
\renewcommand{\Im}{\mathrm{Im}}
\newcommand{\pv}[1]{\mathrm{p.v.}#1} % Cauchy principal value
%\newcommand{\tvector}[2]{\begin{pmatrix}#1\\ #2\end{pmatrix}}
\newcommand{\pmat}[1]{\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\comp}[1]{#1^\complement}

%---------- Symbols -----------------
\renewcommand{\triangle}{\vartriangle}
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\rho}{\varrho}
\renewcommand{\phi}{\varphi}
%\renewcommand{\theta}{\vartheta}
%\renewcommand{\leq}{\leqslant}
%\renewcommand{\geq}{\geqslant}
\newcommand{\fourier}[1]{(#1)^\wedge}
\newcommand{\ifourier}[1]{(#1)^\vee}
%\renewcommand{\hat}{\widehat}
\renewcommand{\bar}[1]{\overline{#1}}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\deg}{$^{\circ}${ }}

\newcommand{\zb}{z.\,B.~} 
\newcommand{\Dh}{D.\,h.~}
\newcommand{\dhh}{d.\,h.~}


\renewcommand{\labelitemi}{$\blacktriangleright$}
\renewcommand{\labelitemii}{$\cdot$}
\renewcommand{\labelitemiii}{$\diamond$}
\renewcommand{\labelitemiv}{$\ast$}

%------------------------------------

%------ Function Spaces ------
% \def\LR{L^1(\R)}
% \def\LsqR{L^2(\R)}
% \def\LsqRw{L^2\left(\R^2,\frac{da db}{a^2}\right)}
\newcommand{\Lp}[2]{L^{#1}(\R^{#2})}

%----------- Equations --------------------------
% \def\eqa{\begin{equation}}
% \def\eqe{\end{equation}}
% \def\eqna{\begin{equation*}}
% \def\eqne{\end{equation*}}
% \def\eqnarraya{\begin{eqnarray}}
% \def\eqnarraye{\end{eqnarray}}
% \def\eqnarrayna{\begin{eqnarray*}}
% \def\eqnarrayne{\end{eqnarray*}}
%------------------------------------------------

% TODO: \addchap funktioniert, es kommt jedoch eine Warnung
% --> spter evtl. wieder aendern
% Obsolete: use \addchap, \addsec instead!
% \newcommand{\nonumberchapter}[1]{%
% 	\chapter*{#1}%
% 	\addcontentsline{toc}{chapter}{#1}%
% }

% My marks
\newcommand{\jf}[1]{{\color{red}#1}}
\newcommand{\todomark}{{\marginpar{\color{blue}TODO}}}

\usepackage{xcolor}
\definecolor{darkblue}{rgb}{0.1,0.1,0.65}
\definecolor{darkgreen}{rgb}{0.1,0.65,0.1}
\definecolor{darkred}{rgb}{0.65,0.1,0.1}
%\definecolor{mybrown}{rgb}{1,0.83,0.61}
%\definecolor{mylightblue}{rgb}{0.73,0.83,0.93}
%\definecolor{mybrown}{cmyk}{0,0.05,0.3,0.01}
%\definecolor{mylightblue}{cmyk}{0.3,0.01,0.01,0}


\definecolor{myblue}{rgb}{.95, .95, 1}
\definecolor{myred}{rgb}{0.975, .95, .95}
\newcommand{\dred}[1]{{\color{darkred}#1}}
\newcommand{\dgreen}[1]{{\color{darkgreen}#1}}
\newcommand{\dblue}[1]{{\color{darkblue}#1}}
\newcommand{\bdred}[1]{{\color{darkred}\textbf{#1}}}
\newcommand{\bdgreen}[1]{{\color{darkgreen}\textbf{#1}}}
\newcommand{\bdblue}[1]{{\color{darkblue}\textbf{#1}}}
